Uhlmann fidelities from tensor networks

Given two states $|\psi\rangle$ and $|\phi\rangle$ of a quantum many-body system, one may use the overlap or fidelity $|\langle\psi|\phi\rangle|$ to quantify how similar they are. To further resolve the similarity of $|\psi\rangle$ and $|\phi\rangle$ in space, one can consider their reduced density matrices $\rho$ and $\sigma$ on various regions of the system, and compute the Uhlmann fidelity $F(\rho, \sigma) = \operatorname{Tr} \sqrt{\sqrt{\rho} \sigma \sqrt{\rho}}$. In this paper, we show how computing such subsystem fidelities can be done efficiently in many cases when the two states are represented as tensor networks. Formulated using Uhlmann's theorem, such subsystem fidelities appear as natural quantities to extract for certain subsystems for Matrix Product States and Tree Tensor Networks, and evaluating them is algorithmically simple and computationally affordable. We demonstrate the usefulness of evaluating subsystem fidelities with three example applications: studying local quenches, comparing critical and non-critical states, and quantifying convergence in tensor network simulations.

==> makefile <==
all: uhlmann.pdf

########################################################################

uhlmann: uhlmann.pdf

uhlmann.pdf: uhlmann.tex uhlmann.bbl
	pdflatex uhlmann.tex
	pdflatex uhlmann.tex

uhlmann.bbl: uhlmann.bcf uhlmann.bib
	bibtex uhlmann

uhlmann.bcf: uhlmann.tex
	pdflatex uhlmann.tex

########################################################################

clean_all: clean
	rm -f uhlmann.pdf

clean: clean_uhlmann

clean_uhlmann:
	rm -f uhlmann.bbl uhlmann.blg uhlmann.log uhlmann.out\
		uhlmann.toc uhlmann.aux uhlmann.bcf\
		uhlmann-blx.bib uhlmann.run.xml uhlmann.tex.blg\
		uhlmann.bib.bak uhlmannNotes.bib

